First Measurement of the Charged Current $\overline{\nu}_{\mu}$ Double Differential Cross Section on a Water Target without Pions in the final state

This paper reports the first differential measurement of the charged-current $\overline{\nu}_{\mu}$ interaction cross section on water with no pions in the final state. The unfolded flux-averaged measurement using the T2K off-axis near detector is given in double differential bins of $\mu^+$ momentum and angle. The integrated cross section in a restricted phase space is $\sigma=\left(1.11\pm0.18\right)\times10^{-38}$ cm$^{2}$ per water molecule. Comparisons with several nuclear models are also presented.

==> fitting-b.tex <==
The cross section, integrated over all kinematic variables is,
\begin{equation}
\sigma=(N_{sel,data}-B)/\epsilon\phi T
\end{equation}

where the variables are the number of selected and reconstructed data
signal events $N_{sel,data}$, the number of background events $B$
determined from the MC, the reconstruction efficiency $\epsilon$,
the neutrino flux per unit area $\phi$, and the number of target
nuclei $T$. The efficiency is determined from Monte Carlo simulation
as
\begin{equation}
\epsilon=(N_{sel,MC}-B)/N_{gen}
\end{equation}

where the number of selected and reconstructed signal MC events is
$N_{sel,MC}$ and the number of generated signal events is $N_{gen}$. 

A differential cross section $\Delta\sigma$ in a particular muon
momentum bin $\Delta p$ and muon angle bin $\Delta cos\theta$ is
given as, 
\begin{equation}
\frac{\Delta\sigma}{\Delta p\Delta cos\theta}=\frac{\Delta N_{sel,data}-B}{\epsilon\left(p,cos\theta\right)\phi T}.
\end{equation}

This assumes the detector reconstruction was perfect, with no momentum
or angle smearing. Lets assume that in a particular $p-cos\theta$
bin $j$ , we find $N_{j}^{sig}$ signal events and the MC predicted,
$N_{j}^{sig,MC}$events. We then determine a fitting coefficient,
$c_{j}$, where,
\begin{equation}
N_{j}^{sig}=c_{j}N_{j}^{sig,MC}
\end{equation}

If we allow for $k$ different backgrounds in the observed data, $\sum_{k}^{bkgd\_types}N_{j}^{bkgd\_k,MC}$,
this could be added to the above equation. In addition if the backgrounds
depend different model parametrization the background can be multiplied
by $\prod_{a}^{model}\omega\left(\vec{a}\right)_{j}^{k}$ which depends
on a vector, $\vec{a}$, parameter. Then the expression becomes,
\begin{equation}
N_{j}=c_{j}N_{j}^{sig,MC}+\sum_{k}^{bkgd\_types}N_{j}^{bkgd\_k,MC}\prod_{a}^{model}\omega\left(\vec{a}\right)_{j}^{k}
\end{equation}

In real experiments the reconstruction is not perfect and we need
to include smearing where events from a particular true $p-cos\theta$
bin $j$ were smeared over several different reconstructed $p-cos\theta$
 bins. Lets consider a generated true $p-cos\theta$ bin $i$ and
the reconstructed bins $j$ where the true kinematic values were possibly
smeared over several $j$ bins. A ``smearing matrix'' $S_{ij}$
can be constructed defined as,
\begin{equation}
S_{ij}=\frac{N_{reco\_in\_j}^{true\_in\_i}}{N^{true\_in\_i}}
\end{equation}

where the true kinematic events in bin $i$ are smeared into bins
$j$. In practice the generated signal appears in bin $i$ and the
reconstructed (or observed) events appears in bin $j$. Then the equation
for the true number of events in bin $i$ in terms of the observed
events in bin $j$ becomes,

\begin{eqnarray}
N_{i} & = & \sum_{j}^{N_{bin}}\{c_{j}N_{j}^{sig,MC}\\
 &  & +\sum_{k}^{bkgd\_types}N_{j}^{bkgd\_k,MC}\prod_{a}^{model}\omega\left(\vec{a}\right)_{j}^{k}\}S_{ij}\nonumber 
\end{eqnarray}

where $j=1,...,N_{bin}$. In this approach{[}Ref. Steve Dolan paper{]}
we have $unfolded$ the true parameters from the observed data. At
this point, using a histogram of observed reconstructed events $N_{i}^{obs}$,
we can form the statistical likelihood\cite{Cousins} {[}baker-cousins
ref{]} as

\begin{equation}
\chi_{stat}^{2}=\sum_{i}^{bins}2\left(N_{i}(\vec{c})-N_{i}^{obs}+N_{i}^{obs}ln\left(\frac{N_{i}^{obs}}{N_{i}(\vec{c})}\right)\right)\label{eq:chisq-stat}
\end{equation}

as a function of the fit parameters $c_{j}$ and model parameters
$\vec{a}$. In addition a penalty term is added to Eqn.(\ref{eq:chisq-stat}),
\begin{equation}
\chi_{bkdg\_model}^{2}(\vec{a})=\left(\vec{a}-\vec{a}{}_{prior}\right)\left[V_{cov}^{model}\right]^{-1}\left(\vec{a}-\vec{a}_{prior}\right)^{T}\label{eq:chi-bkgd}
\end{equation}
 

where $V_{cov}^{model}$ is a covariance matrix containing the uncertainties
and correlated errors on the background model parameters $\vec{a}$
and $\vec{a}_{prior}$ is the initial parameter value.

The number of observed events also includes a the flux term that is
the sum of neutrinos. This has been modeled over the different neutrino
energies as,
\begin{equation}
\sum_{n}^{E_{\nu}}f_{n}^{i}
\end{equation}
 

where $f_{n}^{i}$ is the fraction of nth flux energy bin for reconstructed
bin $i$. This sums to unity. The flux uncertainty is given in a covariance
matrix $V_{cov}^{flux}$ and this adds to Eqn.(\ref{eq:chisq-stat})
the flux penalty term,

\begin{equation}
\chi_{flux\_model}^{2}(\vec{f})=\left(\vec{f}-\vec{f}{}_{prior}\right)\left[V_{cov}^{flux}\right]^{-1}\left(\vec{f}-\vec{f}_{prior}\right)^{T}\label{eq:chisq-flux}
\end{equation}

Finally the detector systematic uncertainties are given in a third
covariance matrix, $V_{cov}^{det}$, with $\vec{r}$ parameters which
vary the reconstructed event rate in bin $i$. This adds the last
penalty term given as, 
\begin{equation}
\chi_{det\_model}^{2}(\vec{a})=\left(\vec{r}-\vec{r}{}_{prior}\right)\left[V_{cov}^{det}\right]^{-1}\left(\vec{r}-\vec{r}_{prior}\right)^{T}\label{eq:chisq-det}
\end{equation}

The experiment took data with fillable water bags and about half data
was taken with water filled bags and the other have with empty bags.
So there were two sets of data types, water-in and and water-out.
So we can fit $N_{bin}$ $p-cos\theta$ bins of water-in data and
$N_{bin}$ $p-cos\theta$ bins of water-out data. The fit parameters
will now include $c_{j}$ for water-in and for $d_{j}$ water-out.
The final equation becomes

\begin{align}
N_{i}= & \sum_{j}^{2N_{bin}}[c_{j}N_{j}^{sig,water-in,MC}+\label{eq:N_i-prediction}\\
 & +d_{j}N_{j}^{sig,water-out,MC}\nonumber \\
 & +\left(\sum_{k}^{bkgd\_types}N_{j}^{bkgd\_k,MC}\right)\nonumber \\
 & \times\prod_{a}^{model}\omega\left(\vec{a}\right)_{j}^{k}]S_{ij}r_{i}\left(\sum_{n}^{E_{\nu}}f_{n}^{i}\right)\nonumber 
\end{align}
where the water-in data corresponds to $j=1,\,N_{bin}$ and the water-out
data corresponds to $j=N_{bin}+1,2N_{bin}$ where $c_{j}=0$ since
no water is in the bags for this data set. The final chisquare equation
of all terms that will be used to fit the data is,
\begin{eqnarray}
\chi_{total}^{2} & = & \chi_{stat}^{2}(\vec{c},\vec{d},\vec{a},\vec{f},\vec{r})+\chi_{bkdg\_model}^{2}(\vec{a})\nonumber \\
 &  & +\chi_{flux\_model}^{2}(\vec{f})+\chi_{det\_model}^{2}(\vec{r})\label{eq:chisq-total}
\end{eqnarray}

where the fit parameters dependence of each term is made explicit.
Note that ultimately, we are interested in the $\vec{c}$ fit parameters
that will be used to extract the unfolded true differential water
cross section.

